Hadronic and partonic sources of direct photons in relativistic heavy-ion collisions

The direct photon spectra and flow ($v_2$, $v_3$) in heavy-ion collisions at SPS, RHIC and LHC energies are investigated within a relativistic transport approach incorporating both hadronic and partonic phases -- the Parton-Hadron-String Dynamics (PHSD). In the present work, four extensions are introduced compared to our previous calculations: (i) going beyond the soft-photon approximation (SPA) in the calculation of the bremsstrahlung processes $meson+meson\to meson+meson+\gamma$, (ii) quantifying the suppression due to the Landau-Pomeranchuk-Migdal (LPM) coherence effect, (iii) adding the additional channels $V+N\to N+\gamma$ and $\Delta\to N+\gamma$ and (iv) providing predictions for Pb+Pb collisions at $\sqrt{s_{NN}}$ = 2.76 TeV. The first issue extends the applicability of the bremsstrahlung calculations to higher photon energies in order to understand the relevant sources in the region $p_T=0.5-1.5$ GeV, while the LPM correction turns out to be important for $p_T<0.4$ GeV in the partonic phase. The results suggest that a large elliptic flow $v_2$ of the direct photons signals a significant contribution of photons produced in interactions of secondary mesons and baryons in the late (hadronic) stage of the heavy-ion collision. In order to further differentiate the origin of the direct photon azimuthal asymmetry (late hadron interactions vs electromagnetic fields in the initial stage), we provide predictions for the triangular flow $v_3(p_T)$ of direct photons. Additionally, we illustrate the magnitude of the photon production in the partonic and hadronic phases as functions of time and local energy density. Finally, the 'cocktail' method for an estimation of the background photon elliptic flow, which is widely used in the experimental works, is supported by the calculations within the PHSD transport approach.

==> refanswer.tex <==

Dear Editor,

we have revised the manuscript and considerably extended the results
following the suggestions of the referee. Please find the detailed
answer to the referees comments below.

_________________________________________

Editors remarks on the figures:

Figure(s) [2]
     Please use lower case for math function: 'cos'

*Answer:* thank you, we corrected the caption.

Figure(s) [3]
     The figures you have provided have features that are "fuzzy" or
     blurred around the curves, lines, lettering, numbering and/or
     symbols. Please send new figure files with clearer features and
     improved readability.

*Answer:* we have re-drawn the diagrams with the higher resolution, improving the quality.

Figure(s) [5]
     Please add period: 'et al.' (short for Latin: 'et alii').

*Answer:* we have corrected this throughout.

Figure(s) [6]
     Please consider using the journal style for cross references;
     here, initial caps, 'Eq. (29)'. Please beware that the
     'hard-coded' equation number is subject to changes, in case the
     numbering changes during revision (or even in production).

*Answer:* we have adjusted the notation.

Figure(s) [7, 13]
     Figure sublabels should be printed on the figures. The preferred
     form is lowercase letters in parentheses: (a), (b), etc.

*Answer:* we have added the sub-figure labels on the plots throughout.

Figure(s) [13, esp. exponents]
     Please increase the font size (axis labels, axis scale values,
     legend, etc.). Please ensure that all lettering is 2 mm or
     larger (1.5 mm for superscripts and subscripts) after scaling to
     the final publication size. Note that the column width is 8.6 cm
     (twice that amount plus gutter for extra wide figures).

*Answer:* we have increased the fonts on figures wherever subscripts are used.

______________________________________________________________________

Answer to the referee report.

----------------------------------------------------------------------
Report of the Referee -- CD10459/Linnyk
----------------------------------------------------------------------

There is no question that the paper deserves to be published in PRC.
It is a major extension of the PHSD model, which already in its
earlier incarnations was instrumental in the hunt for the explanation
of the "direct photon puzzle", the simultaneous observation of large
yields and azimuthal anisotropies of low pT ("thermal") direct photons
in heavy ion collisions.

The extensions of the PHSD model introduced in this work are well
reasoned and useful. Detailed discussions of which "background"
sources can and cannot be identified experimentally, are most welcome.
For the first time the 3d order coefficient (v3) is also calculated
within the model.

Also, I very much appreciate the fact that currently this is the only
microscopic model of direct photon radiation. Even if PHSD doesn't
explain everything, the sheer existence of this approach, orthogonal
to hydro or fireball expansion scenarios, benefits the field by
keeping our minds open.

Finally, I appreciate the long list of references, a good selection of
the relevant literature, including some very recent publications.

I don't see any flaws in the paper that should necessarily be remedied
before publication. I list below, however, a few suggestions which I
think might make the paper even more useful to the reader.


*Answer:*
We thank the referee for the careful reading of the manuscript and
for the positive evaluation of our work. The comments of the referee
are greatly appreciated. The suggestions of the referee to extend
the paper with additional results and the corrections to the text
lead to an improved manuscript. In particular, we have calculated
 in the new version additionally the
centrality-dependence of the elliptic flow v2 and triangular flow v3
of direct photons both at RHIC and LHC as well as the
time-dependence of the photon yield and the elliptic flow "picked
up" in the QGP. Also, the additional statistics collected has
allowed us to decrease the numerical fluctuations and uncertainties
on many of the other plots. We hope that the referee will find the
paper in the extended version suitable for publication.


Abstract:

"predictions for the triangular flow" -> true, it is still a
prediction for LHC, but not for RHIC...

*Answer:* Thank you, we have rewritten this sentence in the abstract.
Additionally, we have added the PHENIX data on the triangular flow to our plot.

General:

This a long, almost review-type paper. It would be very useful to
include the v2 and v3 calculations for all centralities used by the
experiments. (Also, getting the centrality (in)dependencies right is a
serious additional test of any model.)

*Answer:* Thank you, we have added the new plots with the elliptic and triangular
flow of direct photons at  different centralities as relevant for
the PHENIX and ALICE experiments - see figures 21, 22, 23 and 24 in
the new version of the manuscript.

I'm personally not a big fan of the way theoretical curves are
plotted, although I understand that the random kinks and variations
give some information on uncertainties... The same goal could be
achieved by smoothed curves with added error bands, for instance

*Answer:* We have improved the statistical accuracy of our
calculations, thus obtaining smoother curves. We have drawn the
error bands explicitly on the v2 and v3 plots. On the spectra plots
there are many inter-crossing lines, so we refrained from adding
error bands here, as to keep the figures readable.

p 15: The text says the calculation is for 0-40% Au+Au, but then Fig
11 claims to compare to MB

*Answer:* thank you, we corrected this.

p 16: The abstract (rightly) emphasizes that it is important to
clearly distinguish what is and what isn't subtracted experimentally
when direct photon yields or flow are shown. It would be useful to
write a few explanatory sentences here (it is somewhat discussed
later, for flow).

*Answer:* thank you, we have added a discussion about the various
channels and  which of them are accessed independently by experiment
in the beginning of the 'results' section.

p 18: Fig 13 is very instructive, but a similar figure - yields
(rates) vs time would also be useful since it visualizes how (and
when!) anisotropy is built up.

*Answer:* thank you, we have added an additional figure, which shows the
yield and anisotropy versus time. This figure also directly relates to
your other question below to the pages 20/21 (see our answer below).

Fig 14 I understand that the ALICE data are still preliminary, but the
long verbal comparison in the text (high pT, low pT, discrepancies)
without actually being able to see the points on Fig 14 is confusing.

*Answer:* thank you, we have added the preliminary data of the ALICE
collaboration to the figures of the direct spectra and v2 and of the
inclusive photon v2 at srt_NN=2.76 GeV.

p 19: At the end of the first paragraph a remark on how event plane
angle is calculated in the model would be useful. Experiments
typically use hadrons or a combination of hadrons and photons; what is
happening here? (It is not clear a priori that the two event planes
always coincide!)

*Answer:* thank you for your question. You are right that these two planes
do not coincide. We have extended the paragraph with a clarification
that the event plane was fixed through the hadron-hadron
correlations. The details of the procedure are well described in the
references quoted.

p 19: First column, last two paragraphs - I think at the third reading
I understood exactly what the authors wanted to say, but it wasn't
easy (WA98 flow, direct photons yield, etc.)

*Answer:* we have re-written this paragraph to make it more clear.

p 20: First column, last paragraph "the decay photon v2 is accessed
experimentally". Isn't this a typo (you mean direct photon v2, right?)

*Answer:* Yes, it was a typo, thank you very much for correcting us.

p 20/21:
The reasoning here is a bit shaky (but honest: "we cannot
quantitatively answer...", so it's fine). But precisely here a rate
vs. time plot, suggested earlier, would help a lot.
p 23: "...photon production... in the QGP... localized in the center
of the fireball..." I'm not sure I see where has this exactly been
shown (although might be true!) Fig 13 doesn't seem to prove this.
Maybe the (repeated) plea for a rate vs time plot could help here,
too?

*Answer:* thank you. Indeed, we have added a plot for the qualitative
clarification -- Fig. 17 of the new version, -- which shows that the elliptic
flow of the photons reaches only 0.02 during the plasma phase existence. It also
illustrates that the rate of photon production in the QGP decreases with time.

p 21: As duly emphasized in the text, the centrality dependence of v2
is crucial information (and available in PHSD). Why not include the
full centrality dependence (and comparison) just like it was done for
yields in Fig 12?

*Answer:* thank you. Following your suggestion we have added a figure with the
v2 vs pT at different centralites - Figs. 21 and 22 of the new
version. We have previously published the PHSD predictions for the
direct photon v2 at RHIC at different centralities in Phys.Rev. C89
(2014) 3, 034908. In the present plot, we have added the now
available PHENIX data on top of our calculations.

p 22: It has been suggested elsewhere that v2/v3 of photons is
sensitive to eta/s. While this is not hydro, the reader may wonder
what's the prediction of PHSD to this v2/v3 ratio?

*Answer:* It is indeed suggested in hydrodynamics calculations that
the v2/v3 is varying with the variation of the used eta/s. To our
knowledge, this ratio for the direct photons was discussed in
relation to the eta/s variation by U.W. Heinz, J. Liu and C. Shen,
in arXiv:1403.8101. In the scope of the PHSD it is however difficult
to pose such a question. The sheer viscosity in our approach depends
on the interplay of many cross sections of partonic and hadronic
interactions and it is not an adjustable parameter. Such an
investigation is beyond the scope of the current work.

Also, centrality dependence of v3 would also be interesting (it should
be calculable)

*Answer:* yes, thank you, we have calculated the triangular flow coefficients for different
centralities both at RHIC and LHC energies, see Figs. 23 and 24
of the new version of the manuscript.

"triangular flow... PHENIX ... in line with the PHSD calculations" one
more reason to actually show the comparisons (centrality dependence
included)

*Answer:* thank you, we have added the PHENIX data on the v3 plots.

Finally, while thorough proof-reading will obviously follow, a few
wording problems I spotted:

p 1: "possibly production of Glasma" -> "possible production..."
"minimal bias" -> "minimum bias" (throughout the paper)

*Answer:* thank you for noting this, we have corrected.

p 9: "agrees with the 'exact' cross very well" -> "cross section"

*Answer:* thank you for noting this, we have corrected.

p 10: "in stead of (18)" -> "instead of (18)"

*Answer:* thank you for noting this, we have corrected.

p 13: "spacial" -> "spatial"

*Answer:* thank you for noting this, we have corrected.

p 15: "Monitz" -> "Moniz" (In the references it is correct.)

*Answer:* thank you for noting this, we have corrected.

p 19: small inconsistency: the two scenarios are called "scenario a"
and "scenario 2" ...

*Answer:* thank you for noting this, we have corrected.

p 24: "Hedielberg" -> "Heidelberg" (in the references)

*Answer:* thank you for noting this, we have corrected.

